Inferring Streaming Video Quality from Encrypted Traffic: Practical Models and Deployment Experience

Inferring the quality of streaming video applications is important for Internet service providers, but the fact that most video streams are encrypted makes it difficult to do so. We develop models that infer quality metrics (\ie, startup delay and resolution) for encrypted streaming video services. Our paper builds on previous work, but extends it in several ways. First, the model works in deployment settings where the video sessions and segments must be identified from a mix of traffic and the time precision of the collected traffic statistics is more coarse (\eg, due to aggregation). Second, we develop a single composite model that works for a range of different services (i.e., Netflix, YouTube, Amazon, and Twitch), as opposed to just a single service. Third, unlike many previous models, the model performs predictions at finer granularity (\eg, the precise startup delay instead of just detecting short versus long delays) allowing to draw better conclusions on the ongoing streaming quality. Fourth, we demonstrate the model is practical through a 16-month deployment in 66 homes and provide new insights about the relationships between Internet "speed" and the quality of the corresponding video streams, for a variety of services; we find that higher speeds provide only minimal improvements to startup delay and resolution.

==> related.tex <==
\section{Related Work}

Previous work has thoroughly explored video quality, as well as how different
video quality metrics relate to user quality of
experience~\cite{videoQoEsurvey}.  The methods to monitor these metrics,
however, vary according to the vantage point.  Streaming providers can
directly instrument the player to report video
quality~\cite{dobrian2011understanding,
krishnan2013video,balachandran2013developing, ahmed2017suffering}, but one
cannot directly measure quality from within the network.  Therefore, ISPs must
infer video quality based on the observation of the packets traversing the
network. A variety of approaches have been developed for modeling one or more
video quality metrics or quality of experience from network
characteristics~\cite{chen2009oneclick,stuhlmuller2000analysis,
reibman2004quality, tao2008real, venkataraman2011inferring}. These models
pre-date the wide-adoption of DASH. Hence, in practice, ISPs mostly rely on
deep-packet inspection to identify video sessions within network traffic and
then extract video
quality~\cite{sandvineDPI,mangla2017mimic,trevisan2016impact}, which is
becoming infeasible due to encryption of video
sessions~\cite{gsma2015,dyer2015}. This is one of the main challenges we
address in this paper.

Several previous studies infer video quality from encrypted video traffic, as
we do. Dimopoulos \ea~\cite{dimopoulos2016measuring} developed a method that
runs on a web proxy in the network to infer quality of YouTube sessions. Their
study only focuses on YouTube over TCP, so it is unclear whether the methods
generalize to other video services or even to YouTube over QUIC (which is
soaring at astonishing pace~\cite{MVI}). Second, they infer video quality
metrics such as rebuffering, bitrate switches, and the average quality of full
sessions, which is too coarse for some use cases such as online monitoring and
optimization. Finally, the use of a web proxy raises privacy concerns.
eMIMIC~\cite{manglaemimic} improves on the accuracy of Dimopoulos
\ea~\cite{dimopoulos2016measuring}.  The method relies on video segment
detection to build parametric models of video session properties that
translate into quality metrics. eMIMIC was evaluated for two undisclosed video
services, and the model parameters had to be fine-tuned per service.  Our work
provides finer-grained inference targets and work per time slot on data and
models that we intend to release.

Our approach of inferring video quality for each individual time slot is most
similar work from Mazhar and Shafiq~\cite{infocomPaper},
BUFFEST~\cite{krishnamoorthi2017buffest} and
Requet~\cite{gutterman2019requet}.  BUFFEST~\cite{krishnamoorthi2017buffest}
focuses only on rebuffering detection for YouTube. It introduces the method to
identify video segments from encrypted traffic that we leverage to compute
application-layer features. BUFFEST implements a buffer level estimation
emulator. It combines the estimated buffer levels with network layer metrics
to feed a machine learning model and predict the presence of rebuffering at
periodic time slots.  Requet~\cite{gutterman2019requet} extends the video
segment detection method to develop random forest models that infer potential
buffer anomalies and resolution at each segment download. Similarly to
BUFFEST, Requet~\cite{gutterman2019requet} solely focus on YouTube and our
results outperform Requet's resolution inference.  Mazhar and
Shafiq~\cite{infocomPaper} use decision trees to detect rebuffering events in
real-time, whether video quality is high or low, and whether the video session
has started or not. They only evaluate their  model for YouTube (although both
for HTTPS and QUIC), and our evaluation~\cite{bronzino2019network} shows that
it does not  generalize to the other video services we tested. Their models
take as input network- and transport-level features, which add a level of
indirection to video quality. Our work demonstrates that the use of input
features computed over video segments can outperform transport features
reducing the collection cost for the operator. Moreover, our reliance on video
segments helps generalize the method for different transport protocols and
video services because we are removing transport overhead and any differences
in the mapping of segments into packets.  

In contrast to all previous work, we have tested our models in a long-running
deployment. In doing so, we faced a new set of challenges that are not faced
by offline models that can operate on curated traces in controlled lab
settings. More generally, we believe that our work demonstrates the value not
just in testing a model in a controlled setting, but in designing for
operational deployment, which comes with a unique set of challenges.

